Condorcet's Jury Theorem with Abstention

The well-known Condorcet's Jury theorem posits that the majority rule selects the best alternative among two available options with probability one, as the population size increases to infinity. We study this result under an asymmetric two-candidate setup, where supporters of both candidates may have different participation costs. When the decision to abstain is fully rational i.e., when the vote pivotality is the probability of a tie, the only equilibrium outcome is a trivial equilibrium where all voters except those with zero voting cost, abstain. We propose and analyze a more practical, boundedly rational model where voters overestimate their pivotality, and show that under this model, non-trivial equilibria emerge where the winning probability of both candidates is bounded away from one. We show that when the pivotality estimate strongly depends on the margin of victory, victory is not assured to any candidate in any non-trivial equilibrium, regardless of population size and in contrast to Condorcet's assertion. Whereas, under a weak dependence on margin, Condorcet's Jury theorem is restored.

==> RelWork.tex <==
\section{ Related Work}
\label{sec:related}
We return to the calculus of voting model.   Recall that this model doesn't adequately explain large turnout observed in real-world elections.  To quote  Fiorina \cite{fiorina1990information} the paradox of voting is so severe that it is \emph{"the paradox that ate rational choice theory".} 
 
 %To quote Fiorina \cite{fiorina1990information} the paradox of voting is "the paradox that ate rational choice theory".  


Many theories offer different explanations for  large turnouts observed in real world elections. For instance, \cite{riker68} propose that voters receive an additional gain---attributed to sense of performing civic duty and/or  any other psychological  gain---from the act of voting. This theory  only provides a partial and sometimes inconsistent explanation of why people vote \cite{Aldrich}. The other explanation attributes the large turnout to   the social benefit drawn by voters. This social benefit  does not diminish even if the size of the electorate is large \cite{edlin2007voting}.


Other models forgo probabilities and the rational expected utility approach altogether and suggest that voters only consider the \emph{possibility} of being pivotal, which depends on the margin and the total number of voters \cite{Ferejohn74,Meir14}. Further, explanations pertaining to sociological and psychological factors \cite{Sabucedo,Harder} and candidate specific characteristics \cite{Kam} also partially explain the turnout. 


%\gan{\begin{itemize}
 %   \item  Though these theories partially explain turnout they do not explain surprises in large elections
%\end{itemize}}


Our model offers a game theoretic explanation to large turnout using boundedly rational pivot probability model. We remark that several such attempts have been made in literature. Perhaps the most noteworthy model is the "rule utilitarian" model given by Harsanyi \cite{Harsanyi77,Harsanyi1980}. This model assumes that the voters prefer a  social welfare maximizing action if everyone else is also rule utilitarian. %Our model, in contrast,  assume agents to maximize their private utility which depends only on the outcome of election. 

%\rmr{trivial equilibrium also emerges in Obratsova et al}
%- Different explanations for }

%\subsection{Outline} \gan{todo}

%When there are few voters, the value of   pivotality  parameter (importance of each vote) is large  drawing votes from even   costly voters. 

    While expected turnout  is a standard parameter that  controls pivotality, controlled experiments on voters' response to poll information show that \emph{strategic}  voting is more frequent when the winning margin is lower~\cite{meir2020strategic,Ferejohn75}.   It is also observed that  while increasing voter population results in a decrease in overall participation, this decrease is very slow and not consistent with standard models of rational voting behaviour \cite{Blais,fairstein2019modeling}. \cite{Blais} observes empirically that the closeness of election inversely affects voter turnout.   %The voters decision to vote crucially  depends on the perceived margin of victory.
~\cite{fairstein2019modeling} show  that voters' actions are more consistent with various heuristics based on the margin than with `rational' utility maximization models. %We therefore  want to understand equilibrium behavior under such `bounded rational' models where voters overestimate their probability to be pivotal.%, at least when the expected voting outcome is a tie.
%\gan{ Alternate theories of turnout and their shortcmoings.... 
   %  Two most prominant themes; strategic voting vs non-strategic behaviour voting 
%    ... Several theories to formalize the gains from voting; we will stick to the rational calculus of voting model }
%\rmr{I'm pretty sure that the idea that voters overestimate their own pivotality is not new. The Local Dominance model is extreme in that the margin completely determines if a voter thinks she is pivotal. Note that LD also induces equilibria with large turnout so we are definitely not the first who tackle this question. I would say that this is more of a justification of our model and that the main question is indeed the second one of winning probabilities. } 



==> rational.tex <==
\section{Rational Voting Model}
Let there are $N$ voters and  each voter $i$ is characterized by tuple $(\pi_{i}, c_i)$. There is a common distribution $F$ on $[0,1]^2$ from which the voters are sampled independently. Here, $\pi_i$ denotes the prior preference of voter $i$. Furthermore, we consider that the voters vote deterministically i.e. voter $i$ votes for candidate $A$ if   $\pi_i \leq 1/2$ and $B$, otherwise. We say that the voter is a supporter of candidate $A$ if he votes for $A$ otherwise he is a supporter of candidate $B$. There is an unknown state of the world denoted by $s \in [0,1]$. Let $Q$ denote the common prior over the states of the world. Furthermore, let $\mathbb{E}[Q] < 1/2$.  This prior is a common knowledge among voters.  Each voter  receives a private signal $\sigma \in \{0,1\}$ such that $\Pr(\sigma=0|s) $ is increasing in $s$.  Each agent decides  whether to vote an whom  based on posterior belief,  pivot probability and cost for voting. Here, a right candidate is the one who 
